Representation Engineering: A Top-Down Approach to AI Transparency

In this paper, we identify and characterize the emerging area of representation engineering (RepE), an approach to enhancing the transparency of AI systems that draws on insights from cognitive neuroscience. RepE places population-level representations, rather than neurons or circuits, at the center of analysis, equipping us with novel methods for monitoring and manipulating high-level cognitive phenomena in deep neural networks (DNNs). We provide baselines and an initial analysis of RepE techniques, showing that they offer simple yet effective solutions for improving our understanding and control of large language models. We showcase how these methods can provide traction on a wide range of safety-relevant problems, including honesty, harmlessness, power-seeking, and more, demonstrating the promise of top-down transparency research. We hope that this work catalyzes further exploration of RepE and fosters advancements in the transparency and safety of AI systems.

==> comments.tex <==
Also, another reason why people think translating values to action is hard is that things like the model exploration tendencies and whatnot make it not pursue the objective but other things that help it learn

Also, we should mention that humans are not instructed to be maximally moral but instead as efficiently as possible achieve maximum reward.

repeat definition of conscience when describing method

say walkthrough people trying to maximize reward and be completionist/get 100\% of the reward

Should Table 1 be converted to a bar plot?  This might be nice just to keep it from being called ``Table 1''




arXiv checklist:
Make Supplementary Materials / Supplementary Material / Appendix consistent
Make method names consistent
check for ``CPMS'' misspelling


Figure 7 needs to be changed to ``Positive'' and ``Negative'' instead of ``Good'' and ``Bad''.

Remember to mention that some games are part of a validation set should people want to use a validation set.






Saved comments
_____________________
Hedge in framework caption and morality annotation writing that 

Keep it grounded & more specific / clear-cut when talking about ethics / conscience. We can all agree that wanton murder is wrong. Focus on extreme cases when setting it up. ``basic sense of right and wrong'' makes reviewers think that everyone agrees on what is right and wrong. The conscience varies, but everyone has a conscience.


For rebuttal, agree with their moral perspectives. Massage them. Make them see that we are on same side.
Make is sound like we have the same ethical outlook as reviewers in the annotation section. When describing CMPS, mention that `clearly there are better algorithms to be made'. Large room for improvement.


hedges: * make it sound like we have the same ethical outlook as reviewers in the annotation section
* when describing the conscience or CMPS, say there are clearly future better algorithms to be made ("large room for improvement")

Dan Hendrycks, 6:04 PM
The environment spells out the consequences of actions for us.
The \emph{pro tanto} valence.
Not always, but generally. Generally, torture is bad, but not necessarily always according to some. Usually it's of a clearly higher tier than hitting someone.

Dan Hendrycks, 6:09 PM
It is bad in a pro tanto sense--namely, it has bad aspects, but it may be outweighed or overrriden.

Dan Hendrycks, 39 min
I think hedging with "save for psychopaths" makes the relativists be less inclined to side with the psychopaths
_____________________


DOUBLE CHECK FIGURE PLACEMENT AND NUMBERING






Related work should be rewritten into three sections.


Q-learning and Q-value aren't italicized in SAC and Jericho papers.











Just call it "object tree", not "complete object tree". People might think, "is there an incomplete object tree? are there multiple types of object tree in Jiminy Cricket?"


inclusive of diverse perspectives
cross-cultural agreement
